Learning Straight Flows: Variational Flow Matching for Efficient Generation

Flow Matching has limited ability in achieving one-step generation due to its reliance on learned curved trajectories. Previous studies have attempted to address this limitation by either modifying the coupling distribution to prevent interpolant intersections or introducing consistency and mean-velocity modeling to promote straight trajectory learning. However, these approaches often suffer from discrete approximation errors, training instability, and convergence difficulties. To tackle these issues, in the present work, we propose \textbf{S}traight \textbf{V}ariational \textbf{F}low \textbf{M}atching (\textbf{S-VFM}), which integrates a variational latent code representing the ``generation overview'' into the Flow Matching framework. \textbf{S-VFM} explicitly enforces trajectory straightness, ideally producing linear generation paths. The proposed method achieves competitive performance across three challenge benchmarks and demonstrates advantages in both training and inference efficiency compared with existing methods.

==> sec/backup.tex <==

\section{Proof}
\label{app_sec:proof}

\noindent
This appendix provides a self-contained development of the analytical objects and proofs
underlying our method. We introduce a \emph{straight, non-intersecting interpolation} $Z$
that is \emph{compatible} with the linear interpolation induced by a given coupling $X$,
and we establish (i) preservation of time marginals, (ii) reduction of convex transport costs,
and (iii) equivalent characterizations of straight (non-intersecting) couplings.
All results are stated and proved without invoking rectified-flow dynamics.

\bigskip
\noindent\textbf{Notation.}
For a random process $Y=\{Y_t\}_{t\in[0,1]}$, we write $\Law(Y_t)$ for its marginal law at time $t$,
and $\E[\cdot]$ for expectation.
For a coupling $(Y_0,Y_1)$ we denote $\Delta^Y:=Y_1-Y_0$ and the linear interpolant
$Y_t=(1-t)Y_0 + t Y_1$.
Conditional expectations such as $\E[\Delta^Y\mid Y_t=x]$ are understood whenever they exist.

\subsection{Preliminaries}

\begin{definition}[Coupling, linear interpolation, and conditional velocity]
Let $(X_0,X_1)$ be any coupling on $\R^d$ with joint density
$\rho(x_0,x_1)=\rho_{0,\phi}(x_0\mid x_1)\,\rho_1(x_1)$.
Define the linear interpolation
\[
X_t=(1-t)X_0+tX_1,\qquad \Delta^X:=X_1-X_0,\qquad t\in[0,1].
\]
The (Flow-Matching) conditional velocity associated with $X$ is
\[
v^X(x,t) \;:=\; \E\!\big[\Delta^X \,\big|\, X_t=x\big],\qquad (x,t)\in \R^d\times[0,1].
\]
\end{definition}

\begin{definition}[Rectifiability of $X$]
We say that $X$ is \emph{rectifiable} if $v^X(\cdot,t)$ is locally bounded for each $t$ and the continuity equation
\[
\partial_t \pi_t + \nabla\!\cdot\!\big(v^X(\cdot,t)\,\pi_t\big) \;=\;0,\qquad \pi_{t=0}=\Law(X_0),
\]
admits a unique (weak) solution $(\pi_t)_{t\in[0,1]}$.
Equivalently, the ODE $\dot Y_t=v^X(Y_t,t)$ admits a unique flow of characteristics.
\end{definition}

\begin{definition}[Non-intersection functional]
For any coupling $(Y_0,Y_1)$ with linear interpolant $Y_t$, define
\[
V\big((Y_0,Y_1)\big) \;:=\; \int_0^1 \E\!\left[\big\|\,\Delta^Y - \E[\Delta^Y \mid Y_t]\,\big\|^2\right]\,dt.
\]
\end{definition}

\begin{lemma}[Non-intersection iff zero conditional variance]
\label{lem:non_intersection_equiv}
For a coupling $(Y_0,Y_1)$ with linear interpolation $Y_t$, the following are equivalent:
\begin{enumerate}
\item For two i.i.d.\ couplings $(Y_0,Y_1)$ and $(Y_0',Y_1')$,
\begin{equation}
\begin{aligned}
\exists t\in(0,1): &(1-t)Y_0+tY_1=(1-t)Y_0'+tY_1' \\
&\mathcal{P}\!\left[(Y_0,Y_1)\neq(Y_0',Y_1')\right]=0.
\end{aligned}
\end{equation}
\item $V\big((Y_0,Y_1)\big)=0$, i.e.\ $\Delta^Y=\E[\Delta^Y\mid Y_t]$ a.s.\ for a.e.\ $t\in(0,1)$.
\end{enumerate}
\emph{Proof.}
$(1)\Rightarrow(2)$: Non-intersection implies the slope $\Delta^Y$ is a.s.\ a measurable function of $(Y_t,t)$, hence $\Var(\Delta^Y\mid Y_t)=0$; integrating over $t$ gives $V=0$.
$(2)\Rightarrow(1)$: If $\Delta^Y=\E[\Delta^Y\mid Y_t]$ a.s., then the slope through any $Y_t$ is a.s.\ unique; two distinct lines cannot share a point at the same time unless they coincide. \qed
\end{lemma}

\subsection{The straight interpolation $Z$}

\begin{definition}[Straight interpolation compatible with $X$]
\label{def:Z}
A process $Z=\{Z_t\}_{t\in[0,1]}$ on the same probability space as $X$ is called a
\emph{straight interpolation compatible with $X$} if:
\begin{itemize}
\item[(Z1)] (\emph{Linear paths}) There exist $(Z_0,Z_1)$ with $Z_t=(1-t)Z_0+tZ_1$ and $\Delta^Z:=Z_1-Z_0$.
\item[(Z2)] (\emph{Non-intersection}) $V\big((Z_0,Z_1)\big)=0$, equivalently $\Delta^Z=\E[\Delta^Z\mid Z_t]$ a.s.\ for a.e.\ $t$.
\item[(Z3)] (\emph{Velocity-field matching}) With $\mu_t:=\Law(Z_t)$,
\[
v^Z(x,t):=\E[\Delta^Z\mid Z_t=x]=v^X(x,t)\quad\text{for $\mu_t$-a.e.\ $x$ and a.e.\ $t\in[0,1]$.}
\]
\item[(Z4)] (\emph{Initialization}) $Z_0=X_0$ a.s.
\end{itemize}
\end{definition}

\begin{remark}[Immediate consequences]
\label{rem:conseq}
From (Z2), $v^Z(Z_t,t)=\Delta^Z$ a.s., hence
\[
Z_1-Z_0=\int_0^1 v^Z(Z_t,t)\,dt.
\]
By (Z3), $v^Z=v^X$ at $\mu_t$-a.e.\ points, so we also have
\[
\Delta^Z = \int_0^1 v^X(Z_t,t)\,dt.
\]
\end{remark}

\subsection{Main results}

\begin{theorem}[Marginal preservation; analogue of D.3]
\label{thm:marginal_preservation}
Assume $X$ is rectifiable and $Z$ satisfies \emph{Definition~\ref{def:Z}}.
Then $\Law(Z_t)=\Law(X_t)$ for all $t\in[0,1]$.
\end{theorem}

\begin{proof}
Let $h\in C_c^1(\R^d)$. Using (Z1) and (Z2),
\[
\frac{d}{dt}\E[h(Z_t)]
=\E[\nabla h(Z_t)^\top \dot Z_t]
=\E[\nabla h(Z_t)^\top \Delta^Z]
=\E[\nabla h(Z_t)^\top v^Z(Z_t,t)].
\]
By (Z3), $v^Z(\cdot,t)=v^X(\cdot,t)$ $\mu_t$-a.e.; therefore
\[
\frac{d}{dt}\E[h(Z_t)] = \E[\nabla h(Z_t)^\top v^X(Z_t,t)].
\]
This shows that $\mu_t:=\Law(Z_t)$ solves the continuity equation
$\partial_t \mu_t+\nabla\!\cdot\!\big(v^X(\cdot,t)\mu_t\big)=0$ with
$\mu_0=\Law(Z_0)=\Law(X_0)$ by (Z4).
By rectifiability of $X$, the solution is unique and equals $\pi_t:=\Law(X_t)$, hence $\mu_t=\pi_t$ for all $t$.
\end{proof}


\begin{theorem}[Convex transport-cost reduction; analogue of D.5] \label{thm:convex_cost}
Under the assumptions of Theorem~\ref{thm:marginal_preservation}, for any convex $c:\R^d\to\R$,
\[
\E\!\left[c(Z_1-Z_0)\right] \;\le\; \E\!\left[c(X_1-X_0)\right].
\]
If $c$ is strictly convex, the inequality is strict unless $V\big((X_0,X_1)\big)=0$.
\end{theorem}

\begin{proof}
From (Z2), $v^Z(Z_t,t)=\Delta^Z$ a.s., so
\[
Z_1-Z_0=\int_0^1 v^Z(Z_t,t)\,dt.
\]
Applying Jensen in time (which is in fact equality here because $v^Z(Z_t,t)$ is pathwise constant), we get
\[
\E\!\left[c(Z_1-Z_0)\right]
\le \int_0^1 \E\!\left[c\big(v^Z(Z_t,t)\big)\right]\,dt.
\]
By (Z3) and Theorem~\ref{thm:marginal_preservation},
\[
\int_0^1 \E\!\left[c\big(v^Z(Z_t,t)\big)\right]dt
= \int_0^1 \E\!\left[c\big(v^X(X_t,t)\big)\right]dt
= \int_0^1 \E\!\left[c\big(\E[\Delta^X\mid X_t]\big)\right]dt.
\]
A second Jensen (conditionally on $X_t$) yields
\[
\E\!\left[c\big(\E[\Delta^X\mid X_t]\big)\right]
\le \E\!\left[\E\!\left[c(\Delta^X)\mid X_t\right]\right]
= \E\!\left[c(\Delta^X)\right].
\]
Combining the inequalities gives the claim. If $c$ is strictly convex, the only potential slack is the conditional Jensen step; equality there holds iff $\Delta^X=\E[\Delta^X\mid X_t]$ a.s., i.e.\ $V\big((X_0,X_1)\big)=0$ by Lemma~\ref{lem:non_intersection_equiv}.
\end{proof}

\begin{corollary}[Quadratic control of transport]
\label{cor:quadratic_control}
With $c(x)=\|x\|^2$,
\[
\E\!\left[\|Z_1-Z_0\|^2\right]\;\le\;\E\!\left[\|X_1-X_0\|^2\right]
=\int_0^1 \E\!\left[\|\dot X_t\|^2\right]\,dt
=\E\!\left[\|\Delta^X\|^2\right].
\]
\emph{Proof.}
The inequality is Theorem~\ref{thm:convex_cost} for $c(x)=\|x\|^2$.
The identities use $\dot X_t=\Delta^X$ for linear interpolation.
\qed
\end{corollary}

\begin{theorem}[Equivalent characterizations of straight couplings; analogue of D.6]
\label{thm:equivalences}
Assume $X$ is rectifiable and let $Z$ satisfy Definition~\ref{def:Z}.
The following statements are equivalent; when they hold we say $(X_0,X_1)$ is a \emph{straight coupling}.
\begin{enumerate}
\item[\textnormal{(i)}] (\emph{Tight cost}) There exists a strictly convex $c$ with
$\E[c(Z_1-Z_0)]=\E[c(X_1-X_0)]$.
\item[\textnormal{(ii)}] (\emph{Endpoint coincidence}) $(Z_0,Z_1)=(X_0,X_1)$ a.s.
\item[\textnormal{(iii)}] (\emph{Pathwise equality}) $Z_t=X_t$ for all $t\in[0,1]$ a.s.
\item[\textnormal{(iv)}] (\emph{Non-intersection for $X$}) $V\big((X_0,X_1)\big)=0$.
\end{enumerate}
\end{theorem}

\begin{proof}
(iii)$\Rightarrow$(ii)$\Rightarrow$(i) is immediate.

(i)$\Rightarrow$(iv): By Theorem~\ref{thm:convex_cost} with strictly convex $c$, equality forces tightness of the conditional Jensen step, hence
$\Delta^X=\E[\Delta^X\mid X_t]$ a.s., i.e.\ $V\big((X_0,X_1)\big)=0$.

(iv)$\Rightarrow$(iii): If $V((X_0,X_1))=0$, then for a.e.\ $t$ we have
$\dot X_t=\Delta^X=v^X(X_t,t)$.
For $Z$, (Z2) and (Z3) give $\dot Z_t=\Delta^Z=v^Z(Z_t,t)=v^X(Z_t,t)$.
Thus both $X$ and $Z$ solve $\dot Y_t=v^X(Y_t,t)$ with the same initial value $Y_0=X_0=Z_0$ (by (Z4)).
Uniqueness (rectifiability) yields $Z\equiv X$.
\end{proof}

\begin{corollary}[One-step exactness in the straight regime]
\label{cor:one_step}
If any (hence all) of the items in Theorem~\ref{thm:equivalences} hold, then along each path
$v^X(X_t,t)\equiv \Delta^X$ is constant in $t$ and the ODE $\dot y_t=v^X(y_t,t)$ integrates in one step:
\[
X_1 \;=\; X_0 + \int_0^1 v^X(X_t,t)\,dt \;=\; X_0 + \Delta^X.
\]
In particular, if $v_\theta\approx v^X$ at training convergence and $V((X_0,X_1))=0$,
one-step generation $x_1 \approx x_0 + v_\theta(x_0,0)$ is exact in the limit.
\end{corollary}

\subsection{Additional remarks (well-posedness and learning)}

\begin{remark}[Well-posedness assumptions]
All proofs require only: (a) $X$ is rectifiable (Definition above), (b) $Z$ satisfies Definition~\ref{def:Z}.
In particular, $Z$ is \emph{not} defined via a rectification ODE; it is a straight, non-intersecting
interpolation whose conditional velocity matches $X$'s at its own marginals and shares the same
initial law. This is sufficient to conclude marginal preservation and cost reduction.
\end{remark}

\begin{remark}[Connection to variational coupling and Flow Matching]
In our learning procedure, the Flow-Matching loss trains $v_\theta$ toward $v^X$,
while the variational objective drives the total time derivative $\frac{d}{dt}v_\theta(X_t,t)$ to zero.
At convergence, this enforces $\Delta^X=\E[\Delta^X\mid X_t]$ and hence $V((X_0,X_1))=0$,
placing us in the straight regime covered by Theorems~\ref{thm:marginal_preservation}--\ref{thm:equivalences}.
\end{remark}






